Look Ma, No Ground Truth! Ground-Truth-Free Tuning of Structure from Motion and Visual SLAM

Evaluation is critical to both developing and tuning Structure from Motion (SfM) and Visual SLAM (VSLAM) systems, but is universally reliant on high-quality geometric ground truth -- a resource that is not only costly and time-intensive but, in many cases, entirely unobtainable. This dependency on ground truth restricts SfM and SLAM applications across diverse environments and limits scalability to real-world scenarios. In this work, we propose a novel ground-truth-free (GTF) evaluation methodology that eliminates the need for geometric ground truth, instead using sensitivity estimation via sampling from both original and noisy versions of input images. Our approach shows strong correlation with traditional ground-truth-based benchmarks and supports GTF hyperparameter tuning. Removing the need for ground truth opens up new opportunities to leverage a much larger number of dataset sources, and for self-supervised and online tuning, with the potential for a data-driven breakthrough analogous to what has occurred in generative AI.

==> sec/eth3d_slam.tex <==
\begin{table*}[t]
    \centering
    \caption{Result on ETH3D SLAM~\cite{Schops_2019_CVPR} dataset. Each row represents the average results on scenes with the same prefix. The proposed system outperforms global SfM baselines by a large margin, and also achieves better results than COLMAP~\cite{schoenberger2016sfm}.}
    % \vspace{-5px}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a
    l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{Recall @ 0.1m} && \multicolumn{4}{c}{AUC @ 0.1m} && \multicolumn{4}{c}{AUC @ 0.5m} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~Theia~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~Theia~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~Theia~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~Theia~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
cables && \cellcolor{tabsecond}76.8 & \cellcolor{tabfirst}88.0 & \cellcolor{tabfirst}88.0 & 68.0 && 59.1 & \cellcolor{tabsecond}60.2 & \cellcolor{tabfirst}76.2 & 56.5 && 77.4 & \cellcolor{tabsecond}82.4 & \cellcolor{tabfirst}85.6 & 70.4 && \cellcolor{tabfirst}103.1 & 339.5 & \cellcolor{tabsecond}195.6 & 2553.4 \\
camera && 2.2 & 26.6 & \cellcolor{tabsecond}32.6 & \cellcolor{tabfirst}34.8 && 2.0 & 12.9 & \cellcolor{tabsecond}21.9 & \cellcolor{tabfirst}24.7 && 2.2 & 26.2 & \cellcolor{tabsecond}30.8 & \cellcolor{tabfirst}33.2 && \cellcolor{tabfirst}1.5 & \cellcolor{tabsecond}5.3 & 10.0 & 196.2 \\
ceiling && 6.4 & 22.8 & \cellcolor{tabfirst}28.7 & \cellcolor{tabsecond}28.6 && 2.9 & \cellcolor{tabsecond}17.0 & \cellcolor{tabfirst}22.3 & 15.3 && 8.2 & 21.7 & \cellcolor{tabfirst}27.4 & \cellcolor{tabsecond}26.3 && \cellcolor{tabsecond}78.3 & \cellcolor{tabfirst}52.6 & 111.0 & 1057.7 \\
desk && 28.0 & \cellcolor{tabsecond}32.2 & \cellcolor{tabfirst}32.3 & 24.4 && 16.0 & \cellcolor{tabfirst}29.2 & \cellcolor{tabsecond}28.5 & 21.1 && \cellcolor{tabsecond}28.6 & \cellcolor{tabfirst}31.6 & \cellcolor{tabfirst}31.6 & 23.7 && 376.2 & \cellcolor{tabsecond}195.3 & \cellcolor{tabfirst}150.0 & 1115.1 \\
einstein && 32.9 & \cellcolor{tabsecond}47.8 & \cellcolor{tabfirst}48.5 & 33.6 && 22.7 & \cellcolor{tabsecond}32.1 & \cellcolor{tabfirst}36.5 & 25.4 && 34.2 & \cellcolor{tabsecond}46.7 & \cellcolor{tabfirst}47.9 & 36.7 && 150.3 & \cellcolor{tabfirst}70.5 & \cellcolor{tabsecond}142.1 & 1230.8 \\
kidnap && \cellcolor{tabsecond}73.1 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 && 63.4 & 62.3 & \cellcolor{tabfirst}70.3 & \cellcolor{tabsecond}68.5 && 71.2 & 71.1 & \cellcolor{tabfirst}72.7 & \cellcolor{tabsecond}72.3 && \cellcolor{tabfirst}114.4 & 356.7 & \cellcolor{tabsecond}144.3 & 731.2 \\
large && 35.4 & \cellcolor{tabsecond}48.6 & \cellcolor{tabfirst}49.0 & 44.5 && 18.1 & \cellcolor{tabsecond}37.8 & \cellcolor{tabfirst}45.8 & 20.7 && 33.7 & \cellcolor{tabsecond}46.6 & \cellcolor{tabfirst}48.4 & 43.4 && 91.9 & \cellcolor{tabfirst}60.2 & \cellcolor{tabsecond}77.6 & 983.8 \\
mannequin && 49.1 & \cellcolor{tabsecond}62.2 & \cellcolor{tabfirst}67.4 & 59.3 && 36.7 & 46.5 & \cellcolor{tabfirst}61.4 & \cellcolor{tabsecond}52.8 && 49.1 & \cellcolor{tabsecond}59.7 & \cellcolor{tabfirst}66.4 & 58.4 && \cellcolor{tabsecond}33.5 & \cellcolor{tabfirst}29.7 & 44.3 & 301.2 \\
motion && \cellcolor{tabsecond}18.8 & 16.9 & \cellcolor{tabfirst}39.8 & 17.7 && 11.0 & 11.9 & \cellcolor{tabfirst}22.5 & \cellcolor{tabsecond}12.9 && \cellcolor{tabsecond}23.3 & 19.2 & \cellcolor{tabfirst}45.9 & 19.7 && 859.7 & \cellcolor{tabfirst}109.0 & \cellcolor{tabsecond}788.9 & 9995.1 \\
planar && \cellcolor{tabsecond}30.6 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 12.5 & 97.8 & \cellcolor{tabfirst}98.7 & \cellcolor{tabsecond}98.3 && 38.0 & \cellcolor{tabsecond}99.6 & \cellcolor{tabfirst}99.7 & \cellcolor{tabfirst}99.7 && \cellcolor{tabsecond}313.8 & \cellcolor{tabfirst}167.5 & 533.3 & 2349.7 \\
plant && 77.0 & 89.1 & \cellcolor{tabfirst}93.3 & \cellcolor{tabsecond}92.8 && 62.9 & 75.3 & \cellcolor{tabsecond}82.0 & \cellcolor{tabfirst}82.3 && 77.1 & 88.2 & \cellcolor{tabfirst}93.4 & \cellcolor{tabsecond}92.5 && \cellcolor{tabfirst}21.7 & 35.7 & \cellcolor{tabsecond}28.7 & 202.7 \\
reflective && 12.6 & 16.1 & \cellcolor{tabsecond}22.0 & \cellcolor{tabfirst}26.2 && 6.7 & 9.0 & \cellcolor{tabfirst}12.1 & \cellcolor{tabsecond}9.2 && 16.5 & 23.0 & \cellcolor{tabsecond}31.3 & \cellcolor{tabfirst}33.5 && 721.3 & \cellcolor{tabfirst}118.3 & \cellcolor{tabsecond}434.4 & 6573.9 \\
repetitive && 26.3 & \cellcolor{tabsecond}28.5 & \cellcolor{tabfirst}32.7 & \cellcolor{tabsecond}28.5 && 23.9 & 15.2 & \cellcolor{tabfirst}29.2 & \cellcolor{tabsecond}27.2 && 25.8 & 27.0 & \cellcolor{tabfirst}32.0 & \cellcolor{tabsecond}28.3 && \cellcolor{tabfirst}63.2 & 136.8 & \cellcolor{tabsecond}74.5 & 561.1 \\
sfm && 83.2 & \cellcolor{tabsecond}94.1 & \cellcolor{tabfirst}97.0 & 55.9 && \cellcolor{tabsecond}57.9 & 53.7 & \cellcolor{tabfirst}79.6 & 35.7 && 80.0 & \cellcolor{tabsecond}88.7 & \cellcolor{tabfirst}95.2 & 55.8 && \cellcolor{tabfirst}91.7 & \cellcolor{tabsecond}170.5 & 239.7 & 469.6 \\
sofa && 11.2 & 22.0 & \cellcolor{tabsecond}23.9 & \cellcolor{tabfirst}32.2 && 5.5 & 13.1 & \cellcolor{tabsecond}22.1 & \cellcolor{tabfirst}28.6 && 10.3 & 21.3 & \cellcolor{tabsecond}23.5 & \cellcolor{tabfirst}31.6 && \cellcolor{tabsecond}9.1 & \cellcolor{tabfirst}8.9 & 10.1 & 157.3 \\
table && 79.1 & 93.7 & \cellcolor{tabsecond}94.3 & \cellcolor{tabfirst}99.9 && 68.2 & 69.2 & \cellcolor{tabsecond}84.3 & \cellcolor{tabfirst}95.6 && 76.9 & 89.2 & \cellcolor{tabsecond}92.3 & \cellcolor{tabfirst}99.1 && \cellcolor{tabsecond}182.0 & \cellcolor{tabfirst}97.8 & 221.5 & 2777.7 \\
vicon && 64.6 & \cellcolor{tabsecond}84.2 & \cellcolor{tabfirst}97.0 & 81.1 && 20.4 & \cellcolor{tabsecond}57.1 & \cellcolor{tabfirst}80.5 & 38.9 && 71.7 & \cellcolor{tabsecond}87.6 & \cellcolor{tabfirst}93.7 & 75.0 && \cellcolor{tabsecond}50.9 & 88.2 & \cellcolor{tabfirst}46.2 & 474.8 \\
\midrule
\textit{Average} && 48.2 & \cellcolor{tabsecond}62.8 & \cellcolor{tabfirst}66.4 & 57.9 && 34.9 & 46.0 & \cellcolor{tabfirst}57.0 & \cellcolor{tabsecond}47.6 && 48.6 & \cellcolor{tabsecond}61.1 & \cellcolor{tabfirst}65.7 & 57.9 && \cellcolor{tabsecond}120.8 & \cellcolor{tabfirst}91.8 & 133.5 & 1115.4 \\
      \bottomrule
    \end{tabular}
    }
    \label{tbl:eth3d_slam}
    % \vspace{-3px}
\end{table*}

==> sec/eth3d_slam_full.tex <==
\begin{table*}[]
    \centering
    \caption{Per sequence result for ETH3D SLAM}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{l l c c c a l c c c a l c c c a
    l c c c d
    } \toprule 
        % && \multicolumn{4}{c}{OpenMVG} && \multicolumn{4}{c}{Theia} && \multicolumn{4}{c}{Ours} 
        % && \multicolumn{4}{c}{COLMAP}
        && \multicolumn{4}{c}{Recall @ 0.1} && \multicolumn{4}{c}{AUC @ 0.1} && \multicolumn{4}{c}{AUC @ 0.5} 
        && \multicolumn{4}{c}{Time (s)}
        \\
        \cmidrule{3-6} \cmidrule{8-11} \cmidrule{13-16} \cmidrule{18-21}
        && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} && \tiny{OpenMVG} & \tiny{~~~Theia~~~} & \tiny{GLOMAP} & \tiny{COLMAP} \\  \midrule
cables\_1 && \cellcolor{tabsecond}66.5 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 32.5 & 51.9 & \cellcolor{tabsecond}80.5 & \cellcolor{tabfirst}93.8 && 72.3 & 90.4 & \cellcolor{tabsecond}96.1 & \cellcolor{tabfirst}98.8 && \cellcolor{tabfirst}289.0 & 1001.2 & \cellcolor{tabsecond}549.8 & 7501.8 \\
cables\_2 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabsecond}40.2 && \cellcolor{tabfirst}90.9 & 74.6 & \cellcolor{tabsecond}88.0 & 16.7 && \cellcolor{tabfirst}98.2 & 94.9 & \cellcolor{tabsecond}97.6 & 49.4 && \cellcolor{tabsecond}5.2 & \cellcolor{tabfirst}3.8 & 11.6 & 96.8 \\
cables\_3 && \cellcolor{tabfirst}63.9 & \cellcolor{tabfirst}63.9 & \cellcolor{tabfirst}63.9 & \cellcolor{tabfirst}63.9 && 53.9 & 54.1 & \cellcolor{tabfirst}60.1 & \cellcolor{tabsecond}58.9 && 61.9 & 62.0 & \cellcolor{tabfirst}63.2 & \cellcolor{tabsecond}62.9 && \cellcolor{tabsecond}15.0 & \cellcolor{tabfirst}13.5 & 25.5 & 61.5 \\
camera\_shake\_1 && 6.6 & 36.2 & \cellcolor{tabsecond}44.7 & \cellcolor{tabfirst}46.5 && 6.1 & \cellcolor{tabsecond}18.2 & 17.4 & \cellcolor{tabfirst}22.7 && 6.5 & 36.4 & \cellcolor{tabsecond}40.1 & \cellcolor{tabfirst}43.0 && \cellcolor{tabfirst}1.5 & \cellcolor{tabsecond}3.9 & 6.7 & 74.5 \\
camera\_shake\_2 && - & 20.9 & \cellcolor{tabsecond}24.3 & \cellcolor{tabfirst}51.1 && - & 8.6 & \cellcolor{tabsecond}22.1 & \cellcolor{tabfirst}45.0 && - & 19.0 & \cellcolor{tabsecond}24.0 & \cellcolor{tabfirst}49.9 && - & \cellcolor{tabfirst}9.8 & \cellcolor{tabsecond}19.3 & 511.3 \\
camera\_shake\_3 && - & \cellcolor{tabsecond}22.8 & \cellcolor{tabfirst}28.8 & 6.7 && - & \cellcolor{tabsecond}12.0 & \cellcolor{tabfirst}26.2 & 6.4 && - & \cellcolor{tabsecond}23.2 & \cellcolor{tabfirst}28.2 & 6.6 && - & \cellcolor{tabfirst}2.1 & 3.9 & \cellcolor{tabsecond}2.9 \\
ceiling\_1 && - & \cellcolor{tabfirst}9.3 & \cellcolor{tabfirst}9.3 & \cellcolor{tabfirst}9.3 && - & 8.4 & \cellcolor{tabfirst}8.8 & \cellcolor{tabsecond}8.7 && - & \cellcolor{tabsecond}9.1 & \cellcolor{tabfirst}9.2 & \cellcolor{tabfirst}9.2 && - & \cellcolor{tabfirst}17.2 & \cellcolor{tabsecond}40.5 & 116.9 \\
ceiling\_2 && 12.7 & 36.4 & \cellcolor{tabfirst}48.0 & \cellcolor{tabsecond}47.9 && 5.9 & \cellcolor{tabsecond}25.6 & \cellcolor{tabfirst}35.8 & 21.9 && 16.3 & 34.4 & \cellcolor{tabfirst}45.7 & \cellcolor{tabsecond}43.3 && \cellcolor{tabfirst}78.3 & \cellcolor{tabsecond}87.9 & 181.4 & 1998.6 \\
desk\_3 && \cellcolor{tabsecond}37.9 & \cellcolor{tabfirst}46.3 & \cellcolor{tabfirst}46.3 & 28.2 && 16.7 & \cellcolor{tabfirst}42.0 & \cellcolor{tabsecond}39.8 & 27.6 && 39.8 & \cellcolor{tabfirst}45.4 & \cellcolor{tabsecond}45.0 & 28.1 && \cellcolor{tabsecond}126.5 & 255.1 & \cellcolor{tabfirst}124.3 & 767.5 \\
desk\_changing\_1 && 18.1 & 18.2 & \cellcolor{tabsecond}18.4 & \cellcolor{tabfirst}20.6 && 15.2 & \cellcolor{tabsecond}16.4 & \cellcolor{tabfirst}17.2 & 14.7 && 17.5 & 17.8 & \cellcolor{tabsecond}18.1 & \cellcolor{tabfirst}19.4 && 625.9 & \cellcolor{tabfirst}135.4 & \cellcolor{tabsecond}175.6 & 1462.6 \\
einstein\_1 && \cellcolor{tabfirst}90.4 & 85.8 & \cellcolor{tabsecond}87.6 & 45.4 && \cellcolor{tabfirst}46.9 & 35.1 & \cellcolor{tabsecond}44.4 & 18.0 && \cellcolor{tabfirst}88.5 & 85.8 & \cellcolor{tabsecond}88.0 & 56.8 && \cellcolor{tabsecond}122.6 & \cellcolor{tabfirst}120.2 & 139.0 & 1920.6 \\
einstein\_2 && 39.8 & \cellcolor{tabsecond}77.5 & \cellcolor{tabfirst}78.4 & 23.7 && 18.8 & \cellcolor{tabfirst}51.0 & \cellcolor{tabsecond}49.0 & 11.0 && 52.4 & \cellcolor{tabfirst}75.0 & \cellcolor{tabsecond}74.7 & 34.3 && \cellcolor{tabsecond}263.4 & \cellcolor{tabfirst}180.9 & 472.3 & 4765.7 \\
einstein\_dark && - & \cellcolor{tabsecond}5.6 & \cellcolor{tabfirst}7.0 & 5.0 && - & \cellcolor{tabfirst}3.2 & \cellcolor{tabsecond}2.8 & 2.0 && - & \cellcolor{tabsecond}6.3 & \cellcolor{tabfirst}7.4 & 6.1 && - & \cellcolor{tabfirst}20.4 & \cellcolor{tabsecond}31.2 & 267.8 \\
einstein\_flashlight && - & \cellcolor{tabsecond}17.4 & \cellcolor{tabfirst}19.1 & 17.3 && - & \cellcolor{tabsecond}11.2 & \cellcolor{tabfirst}16.3 & 9.4 && - & 16.2 & \cellcolor{tabfirst}18.5 & \cellcolor{tabsecond}17.2 && - & \cellcolor{tabfirst}36.4 & \cellcolor{tabsecond}84.8 & 739.1 \\
einstein\_..change\_1 && - & \cellcolor{tabfirst}17.8 & \cellcolor{tabfirst}17.8 & \cellcolor{tabsecond}11.6 && - & \cellcolor{tabsecond}16.6 & \cellcolor{tabfirst}17.1 & 11.2 && - & \cellcolor{tabsecond}17.6 & \cellcolor{tabfirst}17.7 & 11.5 && - & \cellcolor{tabfirst}8.3 & \cellcolor{tabsecond}19.4 & 21.0 \\
einstein\_..change\_2 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 93.2 & 89.3 & \cellcolor{tabfirst}96.9 & \cellcolor{tabsecond}96.0 && 98.6 & 97.9 & \cellcolor{tabfirst}99.4 & \cellcolor{tabsecond}99.2 && \cellcolor{tabsecond}64.9 & \cellcolor{tabfirst}27.6 & 86.3 & 388.1 \\
einstein\_..change\_3 && - & \cellcolor{tabsecond}30.3 & 30.0 & \cellcolor{tabfirst}32.0 && - & 18.6 & \cellcolor{tabsecond}29.2 & \cellcolor{tabfirst}30.5 && - & 28.0 & \cellcolor{tabsecond}29.9 & \cellcolor{tabfirst}31.7 && - & \cellcolor{tabfirst}100.1 & \cellcolor{tabsecond}161.5 & 513.7 \\
kidnap\_1 && \cellcolor{tabsecond}73.1 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 & \cellcolor{tabfirst}73.3 && 63.4 & 62.3 & \cellcolor{tabfirst}70.3 & \cellcolor{tabsecond}68.5 && 71.2 & 71.1 & \cellcolor{tabfirst}72.7 & \cellcolor{tabsecond}72.3 && \cellcolor{tabfirst}114.4 & 356.7 & \cellcolor{tabsecond}144.3 & 731.2 \\
large\_loop\_1 && 35.4 & \cellcolor{tabsecond}48.6 & \cellcolor{tabfirst}49.0 & 44.5 && 18.1 & \cellcolor{tabsecond}37.8 & \cellcolor{tabfirst}45.8 & 20.7 && 33.7 & \cellcolor{tabsecond}46.6 & \cellcolor{tabfirst}48.4 & 43.4 && 91.9 & \cellcolor{tabfirst}60.2 & \cellcolor{tabsecond}77.6 & 983.8 \\
mannequin\_1 && 26.8 & \cellcolor{tabsecond}43.1 & \cellcolor{tabfirst}53.2 & 18.8 && 17.5 & 16.3 & \cellcolor{tabfirst}45.8 & \cellcolor{tabsecond}17.7 && 31.2 & \cellcolor{tabsecond}38.0 & \cellcolor{tabfirst}51.7 & 18.6 && \cellcolor{tabsecond}18.6 & 30.0 & \cellcolor{tabfirst}17.7 & 45.4 \\
mannequin\_3 && 23.5 & 34.2 & \cellcolor{tabsecond}35.0 & \cellcolor{tabfirst}41.4 && 21.2 & 13.3 & \cellcolor{tabsecond}32.5 & \cellcolor{tabfirst}38.7 && 23.0 & 30.7 & \cellcolor{tabsecond}34.5 & \cellcolor{tabfirst}40.8 && \cellcolor{tabfirst}10.6 & \cellcolor{tabsecond}13.9 & 16.8 & 72.3 \\
mannequin\_4 && 75.3 & 96.3 & \cellcolor{tabsecond}96.7 & \cellcolor{tabfirst}96.9 && 49.7 & 68.6 & \cellcolor{tabfirst}89.8 & \cellcolor{tabsecond}85.6 && 70.2 & 90.9 & \cellcolor{tabfirst}95.3 & \cellcolor{tabsecond}94.6 && \cellcolor{tabsecond}40.2 & \cellcolor{tabfirst}30.0 & 50.2 & 524.0 \\
mannequin\_5 && 43.4 & 68.9 & \cellcolor{tabsecond}77.3 & \cellcolor{tabfirst}80.2 && 15.9 & 34.1 & \cellcolor{tabfirst}63.9 & \cellcolor{tabsecond}59.8 && 52.5 & 66.4 & \cellcolor{tabsecond}74.6 & \cellcolor{tabfirst}78.0 && \cellcolor{tabsecond}88.0 & \cellcolor{tabfirst}82.4 & 94.2 & 1261.3 \\
mannequin\_7 && 13.9 & 15.2 & \cellcolor{tabfirst}19.6 & \cellcolor{tabsecond}18.3 && 9.0 & 14.6 & \cellcolor{tabfirst}18.0 & \cellcolor{tabsecond}17.8 && 13.8 & 15.1 & \cellcolor{tabfirst}19.3 & \cellcolor{tabsecond}18.2 && \cellcolor{tabsecond}6.8 & \cellcolor{tabfirst}6.2 & 12.5 & 19.7 \\
mannequin\_face\_1 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 92.6 & 97.2 & \cellcolor{tabfirst}98.6 & \cellcolor{tabsecond}98.1 && 98.5 & 99.4 & \cellcolor{tabfirst}99.7 & \cellcolor{tabsecond}99.6 && \cellcolor{tabsecond}40.8 & \cellcolor{tabfirst}17.3 & 49.0 & 248.2 \\
mannequin\_face\_2 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && \cellcolor{tabsecond}98.1 & \cellcolor{tabsecond}98.1 & \cellcolor{tabfirst}99.0 & \cellcolor{tabfirst}99.0 && \cellcolor{tabsecond}99.6 & \cellcolor{tabsecond}99.6 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 && \cellcolor{tabsecond}53.2 & \cellcolor{tabfirst}17.6 & 76.3 & 244.4 \\
mannequin\_face\_3 && 17.4 & 45.2 & \cellcolor{tabfirst}69.5 & \cellcolor{tabsecond}64.3 && 14.9 & 32.5 & \cellcolor{tabfirst}51.9 & \cellcolor{tabsecond}45.1 && 16.9 & 42.7 & \cellcolor{tabfirst}66.1 & \cellcolor{tabsecond}62.3 && \cellcolor{tabfirst}16.8 & \cellcolor{tabsecond}21.7 & 52.4 & 285.6 \\
mannequin\_head && 41.9 & \cellcolor{tabfirst}56.8 & \cellcolor{tabsecond}55.7 & 14.0 && 11.2 & \cellcolor{tabsecond}43.5 & \cellcolor{tabfirst}52.6 & 13.1 && 36.1 & \cellcolor{tabsecond}54.1 & \cellcolor{tabfirst}56.8 & 13.8 && \cellcolor{tabsecond}26.8 & 47.8 & 29.9 & \cellcolor{tabfirst}10.2 \\
motion\_1 && \cellcolor{tabsecond}18.8 & 16.9 & \cellcolor{tabfirst}39.8 & 17.7 && 11.0 & 11.9 & \cellcolor{tabfirst}22.5 & \cellcolor{tabsecond}12.9 && \cellcolor{tabsecond}23.3 & 19.2 & \cellcolor{tabfirst}45.9 & 19.7 && 859.7 & \cellcolor{tabfirst}109.0 & \cellcolor{tabsecond}788.9 & 9995.1 \\
planar\_2 && \cellcolor{tabsecond}24.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 9.2 & \cellcolor{tabsecond}99.0 & \cellcolor{tabfirst}99.1 & \cellcolor{tabfirst}99.1 && \cellcolor{tabsecond}31.8 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 & \cellcolor{tabfirst}99.8 && \cellcolor{tabsecond}330.5 & \cellcolor{tabfirst}149.9 & 540.3 & 1220.9 \\
planar\_3 && \cellcolor{tabsecond}37.2 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 15.7 & 96.7 & \cellcolor{tabfirst}98.3 & \cellcolor{tabsecond}97.5 && 44.2 & 99.3 & \cellcolor{tabfirst}99.7 & \cellcolor{tabsecond}99.5 && \cellcolor{tabsecond}297.1 & \cellcolor{tabfirst}185.1 & 526.3 & 3478.5 \\
plant\_1 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 90.1 & 97.8 & \cellcolor{tabfirst}98.6 & \cellcolor{tabsecond}98.5 && 98.0 & \cellcolor{tabsecond}99.6 & \cellcolor{tabfirst}99.7 & \cellcolor{tabfirst}99.7 && \cellcolor{tabsecond}3.9 & \cellcolor{tabfirst}1.9 & \cellcolor{tabsecond}3.9 & 10.7 \\
plant\_2 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 98.1 & 98.5 & \cellcolor{tabfirst}98.8 & \cellcolor{tabsecond}98.6 && 99.6 & \cellcolor{tabsecond}99.7 & \cellcolor{tabfirst}99.8 & \cellcolor{tabsecond}99.7 && \cellcolor{tabfirst}7.4 & \cellcolor{tabsecond}7.6 & 20.4 & 45.3 \\
plant\_3 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 54.4 & \cellcolor{tabfirst}96.2 & 93.2 & \cellcolor{tabsecond}93.8 && 90.9 & \cellcolor{tabfirst}99.2 & 98.6 & \cellcolor{tabsecond}98.8 && 15.0 & \cellcolor{tabfirst}7.7 & \cellcolor{tabsecond}14.6 & 45.9 \\
plant\_4 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 97.9 & \cellcolor{tabsecond}98.8 & 98.7 & \cellcolor{tabfirst}98.9 && 99.6 & \cellcolor{tabfirst}99.8 & \cellcolor{tabsecond}99.7 & \cellcolor{tabfirst}99.8 && \cellcolor{tabsecond}3.8 & \cellcolor{tabfirst}3.6 & 16.0 & 19.1 \\
plant\_5 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 95.7 & 96.3 & \cellcolor{tabfirst}98.3 & \cellcolor{tabsecond}97.0 && 99.1 & 99.3 & \cellcolor{tabfirst}99.7 & \cellcolor{tabsecond}99.4 && \cellcolor{tabsecond}7.3 & \cellcolor{tabfirst}6.9 & 18.5 & 36.3 \\
plant\_scene\_1 && 43.9 & \cellcolor{tabsecond}77.8 & \cellcolor{tabsecond}77.8 & \cellcolor{tabfirst}98.5 && 36.1 & 52.2 & \cellcolor{tabsecond}71.8 & \cellcolor{tabfirst}85.0 && 42.3 & 72.7 & \cellcolor{tabsecond}76.6 & \cellcolor{tabfirst}95.8 && \cellcolor{tabsecond}35.4 & \cellcolor{tabfirst}25.0 & 39.6 & 441.4 \\
plant\_scene\_2 && 41.6 & \cellcolor{tabsecond}84.4 & \cellcolor{tabfirst}99.0 & 76.1 && 15.8 & 27.8 & \cellcolor{tabfirst}58.3 & \cellcolor{tabsecond}35.5 && 59.2 & \cellcolor{tabsecond}83.4 & \cellcolor{tabfirst}91.3 & 82.3 && 80.4 & \cellcolor{tabfirst}54.2 & \cellcolor{tabsecond}64.8 & 644.6 \\
plant\_scene\_3 && 30.4 & 50.3 & \cellcolor{tabfirst}69.6 & \cellcolor{tabsecond}67.8 && 15.1 & 34.6 & \cellcolor{tabsecond}38.6 & \cellcolor{tabfirst}50.8 && 27.7 & 52.3 & \cellcolor{tabfirst}81.9 & \cellcolor{tabsecond}64.4 && \cellcolor{tabfirst}20.2 & 179.1 & \cellcolor{tabsecond}51.5 & 378.5 \\
reflective\_1 && 12.6 & 16.1 & \cellcolor{tabsecond}22.0 & \cellcolor{tabfirst}26.2 && 6.7 & 9.0 & \cellcolor{tabfirst}12.1 & \cellcolor{tabsecond}9.2 && 16.5 & 23.0 & \cellcolor{tabsecond}31.3 & \cellcolor{tabfirst}33.5 && 721.3 & \cellcolor{tabfirst}118.3 & \cellcolor{tabsecond}434.4 & 6573.9 \\
repetitive && 26.3 & \cellcolor{tabsecond}28.5 & \cellcolor{tabfirst}32.7 & \cellcolor{tabsecond}28.5 && 23.9 & 15.2 & \cellcolor{tabfirst}29.2 & \cellcolor{tabsecond}27.2 && 25.8 & 27.0 & \cellcolor{tabfirst}32.0 & \cellcolor{tabsecond}28.3 && \cellcolor{tabfirst}63.2 & 136.8 & \cellcolor{tabsecond}74.5 & 561.1 \\
sfm\_bench && 72.0 & 96.6 & \cellcolor{tabsecond}98.3 & \cellcolor{tabfirst}100.0 && 61.0 & 88.6 & \cellcolor{tabsecond}92.7 & \cellcolor{tabfirst}94.1 && 69.8 & 95.0 & \cellcolor{tabsecond}97.2 & \cellcolor{tabfirst}98.8 && \cellcolor{tabsecond}73.9 & \cellcolor{tabfirst}41.3 & 103.6 & 461.4 \\
sfm\_garden && 76.4 & 80.0 & \cellcolor{tabfirst}87.8 & \cellcolor{tabsecond}84.7 && \cellcolor{tabsecond}32.5 & 31.1 & \cellcolor{tabfirst}57.2 & 29.4 && 76.6 & 79.7 & \cellcolor{tabfirst}90.3 & \cellcolor{tabsecond}82.3 && \cellcolor{tabfirst}272.8 & \cellcolor{tabsecond}698.3 & 835.2 & 798.1 \\
sfm\_house\_loop && \cellcolor{tabsecond}70.5 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & 42.4 && 53.0 & \cellcolor{tabsecond}76.6 & \cellcolor{tabfirst}86.3 & 31.2 && 67.0 & \cellcolor{tabsecond}95.3 & \cellcolor{tabfirst}97.3 & 40.8 && \cellcolor{tabfirst}95.6 & \cellcolor{tabsecond}96.5 & 222.8 & 1030.1 \\
sfm\_lab\_room\_1 && \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 & \cellcolor{tabfirst}99.6 & \cellcolor{tabsecond}20.9 && \cellcolor{tabsecond}75.7 & 44.0 & \cellcolor{tabfirst}77.9 & 11.7 && \cellcolor{tabsecond}94.8 & 88.5 & \cellcolor{tabfirst}95.3 & 23.5 && \cellcolor{tabfirst}12.8 & \cellcolor{tabsecond}14.3 & 32.1 & 37.9 \\
sfm\_lab\_room\_2 && \cellcolor{tabsecond}97.6 & 94.4 & \cellcolor{tabfirst}99.2 & 31.2 && \cellcolor{tabsecond}67.2 & 28.2 & \cellcolor{tabfirst}84.0 & 12.3 && \cellcolor{tabsecond}91.5 & 84.9 & \cellcolor{tabfirst}96.2 & 33.5 && \cellcolor{tabsecond}3.3 & \cellcolor{tabfirst}2.3 & 5.0 & 20.7 \\
sofa\_1 && 10.6 & 21.3 & \cellcolor{tabsecond}25.9 & \cellcolor{tabfirst}27.0 && 5.7 & 11.7 & \cellcolor{tabsecond}22.9 & \cellcolor{tabfirst}24.1 && 9.6 & 22.1 & \cellcolor{tabsecond}25.3 & \cellcolor{tabfirst}26.4 && \cellcolor{tabfirst}13.3 & 21.1 & \cellcolor{tabsecond}14.1 & 252.8 \\
sofa\_2 && 18.6 & \cellcolor{tabsecond}21.8 & \cellcolor{tabsecond}21.8 & \cellcolor{tabfirst}43.1 && 8.3 & 11.3 & \cellcolor{tabsecond}20.4 & \cellcolor{tabfirst}38.7 && 16.6 & 19.7 & \cellcolor{tabsecond}21.5 & \cellcolor{tabfirst}42.4 && \cellcolor{tabsecond}9.2 & \cellcolor{tabfirst}6.1 & 9.8 & 137.2 \\
sofa\_3 && 15.5 & 19.5 & \cellcolor{tabsecond}22.5 & \cellcolor{tabfirst}28.9 && 8.1 & 15.4 & \cellcolor{tabsecond}21.1 & \cellcolor{tabfirst}25.0 && 14.9 & 20.4 & \cellcolor{tabsecond}22.2 & \cellcolor{tabfirst}28.1 && \cellcolor{tabsecond}4.9 & \cellcolor{tabfirst}2.9 & 5.1 & 50.4 \\
sofa\_4 && - & \cellcolor{tabsecond}25.3 & \cellcolor{tabsecond}25.3 & \cellcolor{tabfirst}29.9 && - & 14.0 & \cellcolor{tabsecond}23.8 & \cellcolor{tabfirst}26.8 && - & 23.2 & \cellcolor{tabsecond}25.1 & \cellcolor{tabfirst}29.3 && - & \cellcolor{tabfirst}5.5 & \cellcolor{tabsecond}11.5 & 188.8 \\
table\_3 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 85.9 & 90.3 & \cellcolor{tabfirst}97.7 & \cellcolor{tabsecond}96.8 && 97.2 & 98.1 & \cellcolor{tabfirst}99.5 & \cellcolor{tabsecond}99.4 && 299.0 & \cellcolor{tabfirst}83.0 & \cellcolor{tabsecond}281.2 & 2116.8 \\
table\_4 && \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 && 89.1 & 88.2 & \cellcolor{tabsecond}95.9 & \cellcolor{tabfirst}96.0 && \cellcolor{tabsecond}97.8 & 97.6 & \cellcolor{tabfirst}99.2 & \cellcolor{tabfirst}99.2 && \cellcolor{tabsecond}142.0 & \cellcolor{tabfirst}68.8 & 182.8 & 2817.7 \\
table\_7 && 37.2 & 81.0 & \cellcolor{tabsecond}83.0 & \cellcolor{tabfirst}99.7 && 29.6 & 29.0 & \cellcolor{tabsecond}59.2 & \cellcolor{tabfirst}94.1 && 35.7 & 72.0 & \cellcolor{tabsecond}78.2 & \cellcolor{tabfirst}98.6 && \cellcolor{tabfirst}104.9 & \cellcolor{tabsecond}141.7 & 200.5 & 3398.7 \\
vicon\_light\_1 && 47.2 & 68.5 & \cellcolor{tabsecond}94.1 & \cellcolor{tabfirst}97.8 && 14.4 & 25.6 & \cellcolor{tabfirst}65.8 & \cellcolor{tabsecond}55.4 && 60.8 & 77.5 & \cellcolor{tabsecond}88.4 & \cellcolor{tabfirst}89.9 && \cellcolor{tabsecond}67.9 & 128.7 & \cellcolor{tabfirst}53.3 & 345.1 \\
vicon\_light\_2 && \cellcolor{tabsecond}82.0 & \cellcolor{tabfirst}100.0 & \cellcolor{tabfirst}100.0 & 64.3 && 26.4 & \cellcolor{tabsecond}88.6 & \cellcolor{tabfirst}95.3 & 22.3 && 82.7 & \cellcolor{tabsecond}97.7 & \cellcolor{tabfirst}99.1 & 60.1 && \cellcolor{tabfirst}33.8 & 47.8 & \cellcolor{tabsecond}39.0 & 604.6 \\
\midrule
\textit{Average} && 48.2 & \cellcolor{tabsecond}62.8 & \cellcolor{tabfirst}66.4 & 57.9 && 34.9 & 46.0 & \cellcolor{tabfirst}57.0 & \cellcolor{tabsecond}47.6 && 48.6 & \cellcolor{tabsecond}61.1 & \cellcolor{tabfirst}65.7 & 57.9 && \cellcolor{tabsecond}120.8 & \cellcolor{tabfirst}91.8 & 133.5 & 1115.4 \\

      \bottomrule
    \end{tabular}
    }
    \label{tbl:eth3d_slam_full}
    % \vspace{-3px}
\end{table*}
